Luminous solar neutrinos II: Mass-mixing portals

Solar neutrinos can be efficiently upscattered to MeV scale heavy neutral leptons (HNLs) within the Earth's mantle. HNLs can then decay to electron-positron pairs leading to energy deposition inside large-volume detectors. In this paper we consider mass-portal upscattering of solar neutrinos to HNLs of mass 20 MeV $\geq m_N \geq 2 m_e$. The large volume of the Earth compensates for the long decay-length of the HNLs leading to observable rates of $N\rightarrow \nu_\alpha e^+e^-$ in large volume detectors. We find that searches for mantle-upscattered HNLs can set the novel limits on mixing with third generation leptons, $|U_{\tau N}|$ for masses in the MeV regime; sensitivity to mixing with first- and second-generation leptons is not competitive with existing search strategies.

==> Commands/flags.tex <==
\newcommand{\roni}[1]{\textcolor{red}{[{\bf RH}: #1]}}
\newcommand{\ryan}[1]{\textcolor{blue}{[{\bf RP}: #1]}}
\newcommand{\hari}[1]{\textcolor{Brown}{[{\bf HR}: #1]}}
\newcommand{\maxim}[1]{\textcolor{ForestGreen}{[{\bf MP}: #1]}}


==> Commands/ryansCommands.tex <==
\newcommand{\citer}[1]{Ref. \cite{#1}}
\def\iu{\mathrm{i}}
\def\e{\mathrm{e}}
\def\Ldet{\ell}
\def\Ldec{\lambda}
